Gas Accretion and Star-Formation Rates with IFUs and Background Quasars

Star-forming galaxies (SFGs) are forming stars at a regular pace, forming the so-called main sequence (MS). However, all studies of their gas content show that their gas reservoir ought to be depleted in 0.5-2 Gyr. Thus, SFGs are thought to be fed by the continuous accretion of intergalactic gas in order to sustain their star-formation activity. However, direct observational evidence for this accretion phenomenon has been elusive. Theoretically, the accreted gas coming from the intergalactic medium is expected to orbit about the halo, delivering not just fuel for star-formation but also angular momentum to the galaxy. This accreting material is thus expected to form a gaseous structure that should be co-rotating with the host once at $r<0.3\;R_{\rm vir}$ or $r<10-30$ kpc. Because of the rough alignment between the star-forming disk and this extended gaseous structure, the accreting material can be most easily detected with the combination of background quasars and integral field units (IFUs). In this chapter, accretion studies using this technique are reviewed.

==> referenc-bouche.tex <==
\begin{thebibliography}{92}

\bibitem[Bacon et al.(2010)]{BaconR_10a}
{Bacon}, R., {Accardo}, M., {Adjali}, L., et al., SPIE, 7735, 8

\bibitem[Bauermeiester et al.(2010)]{BauermeisterA_10a}
{Bauermeister}, A., {Blitz}, L., \& {Ma}, C. 2010, \apj, 717, 323

\bibitem[Bigiel et al.(2010)]{BigielF_10a}
{Bigiel}, F., {Leroy}, A., {Seibert}, M., et al. 2010, \apjl, 720, L31

\bibitem[Birnboim \& Dekel(2003)]{BirnboimY_03a}
{Birnboim}, Y., \& {Dekel}, A. 2003, \mnras, 345, 349

\bibitem[Birnboim et al.(2007)]{BirnboimY_07a}
{Birnboim}, Y., {Dekel}, A., \& {Neistein}, E. 2007 \mnras, 380, 339

\bibitem[Bonnet et al.(2004)]{BonnetH_04a}
{Bonnet}, H., {Conzelmann}, R., {Delabre}, B., et al. 2004, SPIE, 5490, 130

\bibitem[Bordoloi et al.(2011)]{BordoloiR_11a}
{Bordoloi}, R., {Lilly}, S.J., {Knobel}, C., et al. 2011, \apj, 743, 10

\bibitem[Bouch\'e et al.(2010)]{BoucheN_10a}
{Bouch{\'e}}, N., {Dekel}, A., {Genzel}, R., et al. 2010, \apj, 718, 1001

\bibitem[Bouch\'e et al.(2016)]{BoucheN_16a}
{Bouch{\'e}}, N., {Finley}, H., {Schroetter}, I., et al. 2016, \apj, 820, 121 

\bibitem[Bouch\'e et al.(2012)]{BoucheN_12a}
{Bouch{\'e}}, N., {Hohensee}, W., {Vargas}, R., et al. 2012, \mnras, 426, 801

\bibitem[Bouch\'e et al.(2013)]{BoucheN_13a}
{Bouch{\'e}}, N., {Murphy}, M.T., {Kacprzak}, G.G., et al. 2013, Science, 341, 50

\bibitem[Bouch\'e et al.(2012)]{BoucheN_11a}
{Bouch{\'e}}, N., {Murphy}, M.T., {P{\'e}roux}, C., et al. 2012, \mnras, 419, 2

\bibitem[Bouch\'e et al.(2007)]{BoucheN_07a}
{Bouch{\'e}}, N., {Murphy}, M.T., {P{\'e}roux}, C., et al. 2007, \apjl, 669, L5

\bibitem[Brinchmann et al.(2004)]{BrinchmannJ_04a}
{Brinchmann}, J., {Charlot}, S., {White}, S.D.M., et al. 2004, \mnras, 351, 1151

\bibitem[Bullock et al.(2001)]{BullockJ_01a}
{Bullock}, J.S., {Dekel}, A., {Kolatt}, T.S., et al. 2001, \apj, 555, 240

%\bibitem[Cantalupo(2017)]{CantalupoS_Springer}
%{Cantalupo}, S.: in {\it Gas Accretion onto Galaxies}, 
%Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion and Lyman-alpha blobs, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Chen et al.(2010)]{ChenY_10a}
{Chen}, Y., {Tremonti}, C.A., {Heckman}, T.M., et al. 2010, \aj, 140, 445

\bibitem[Crighton et al.(2015)]{CrightonN_15a}
{Crighton}, N.H.M., {Murphy}, M.T., {Prochaska}, J.X., et al. 2015, \mnras, 452, 217

\bibitem[Daddi et al.(2007)]{DaddiE_07a}
{Daddi}, E., {Dickinson}, M., {Morrison}, G., et al. 2007, \apj, 670, 156 

\bibitem[Danovich et al.(2015)]{DanovichM_15a}
{Danovich}, M., {Dekel}, A., {Hahn}, O., {Ceverino}, D., {Primack}, J. 2015, 
\mnras, 449, 2087

\bibitem[Danovich et al.(2012)]{DanovichM_12a}
{Danovich}, M., {Dekel}, A., {Hahn}, O., {Teyssier}, R. 2012, \mnras, 442, 1732

\bibitem[Dav\'e et al.(2012)]{DaveR_12a}
{Dav{\'e}}, R., {Finlator}, K., {Oppenheimer}, B.D.: 2012, \mnras, 421, 98

\bibitem[Dekel \& Birnboim(2006)]{DekelA_06a}
{Dekel}, A., {Birnboim}, Y. 2006, \mnras, 368, 2

\bibitem[Dekel et al.(2009)]{DekelA_09a}
{Dekel}, A., {Birnboim}, Y., {Engel}, G., et al. 2009, Nature, 457, 451

\bibitem[Dekel \& Mandelker(2014)]{DekelA_14a}
{Dekel}, A., \& {Mandelker}, N. 2014, \mnras, 444, 2071

\bibitem[Dekel et al.(2013)]{DekelA_13a}
{Dekel}, A., {Zolotov}, A., {Tweed}, D., et al. 2013, \mnras, 435, 999

\bibitem[Elbaz et al.(2007)]{ElbazD_07a}
{Elbaz}, D., {Daddi}, E., {Le Borgne}, D., et al. 2007, \aap, 468, 33

%\bibitem[Faucher-Gigu\`ere(2017)]{Faucher-Giguere_Springer}
%{Faucher-Gig\`uere}, C.A.: in {\it Gas Accretion onto Galaxies}, 
%Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion diagnostics in absorption and emission, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Faucher-Gigu\`ere(2011)]{FaucherG_11b}
{Faucher-Gigu{\`e}re}, C.A., {Kere{\v s}}, D., \& {Ma}, C.P. 2011, \mnras, 417, 2982

\bibitem[Feldmann(2013)]{FeldmannR_13a}
{Feldmann}, R. 2013, \mnras, 433, 1910

\bibitem[Feldmann(2015)]{FeldmannR_15a}
{Feldmann}, R. 2015, \mnras, 449, 3274 

\bibitem[Forbes et al.(2014)]{ForbesJ_14a}
{Forbes}, J.C., {Krumholz}, M.R., {Burkert}, A., {Dekel}, A. 2014, \mnras, 438, 1552

\bibitem[F\"orster Schreiber et al.(2009)]{ForsterSchreiberN_09a}
{F{\"o}rster Schreiber}, N.M., {Genzel}, R., {Bouch{\'e}}, N., et al. 2009, \apj, 706, 1364 

\bibitem[F\"orster Schreiber et al.(2006)]{ForsterSchreiberN_06a}
{F{\"o}rster Schreiber}, N.M., {Genzel}, R., {Lehnert}, M.D., et al. 2006, \apj, 645, 1062 

\bibitem[Freundlich et al.(2013)]{FreundlichJ_13a}
{Freundlich}, J., {Combes}, F., {Tacconi}, L. J., et al. 2013, \aap, 553, A130 

\bibitem[Fumagalli et al.(2011)]{FumagalliM_11a}
{Fumagalli}, M., {Prochaska}, J.X., {Kasen}, D., et al. 2011, \mnras, 418, 1796

\bibitem[Genel et al.(2008)]{GenelS_08a}
{Genel}, S., {Genzel}, R., {Bouch{\'e}}, N., et al. 2008, \apj, 688, 789 

\bibitem[Genzel et al.(2010)]{GenzelR_10a}
{Genzel}, R., {Tacconi}, L.J., {Gracia-Carpio}, J., et al. 2010, \mnras, 407, 2091 

\bibitem[Goerdt et al.(2012)]{GoerdtT_12a}
{Goerdt}, T., {Dekel}, A., {Sternberg}, A., {Gnat}, O., \& {Ceverino}, D. 2012, \mnras, 424, 2292 

\bibitem[Huchtmeier \& Bohnenstengel(1981)]{HuchtmeierW_81a}
{Huchtmeier}, W. K., {Bohnenstengel}, H. D. 1981, \aap, 100, 72

%\bibitem[Kacprzak(2017)]{KacprzakG_Springer}
%{Kacprzak}, G.: in {\it Gas Accretion onto Galaxies}, Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion in star-forming galaxies, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Kacprzak(2012)]{KacprzakG_12a}
{Kacprzak}, G.G., {Churchill}, C.W., {Nielsen}, N.M.: et al. 2012, \apjl, 760, L7 

%\bibitem[Kere\v{s}(2017)]{KeresD_Springer}
%{Kere\v{s}}, D., in {\it Gas Accretion onto Galaxies}, Astrophysics and Space Science
%  Library, vol.~vv, p.~xx,
%chap. Gas accretion within galaxy halos, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Kere\v{s} et al.(2005)]{KeresD_05a}
{Kere\v{s}}, D., {Katz}, N., {Weinberg}, D.H., \& {Dav{\'e}}, R. 2005, \mnras, 363, 2 

\bibitem[Kimm et al.(2011)]{KimmT_11b}
{Kimm}, T., {Devriendt}, J., {Slyz}, A., et al. 2011, preprint, arXiv:1106.0538

\bibitem[Krumholz et al.(2012)]{KrumholzM_12a}
{Krumholz}, M.R., {Dekel}, A., \& {McKee}, C.F. 2012, \apj, 745, 

\bibitem[Lanzetta \& Bowen(1990)]{LanzettaK_90a}
{Lanzetta}, K.M., {Bowen}, D.: 1990, \apj, 357, 321

%\bibitem[Lehner(2017)]{LehnerN_Springer}
%{Lehner}, N.: in {\it Gas Accretion onto Galaxies}, Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion via Lyman Limit Systems, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Leroy et al.(2008)]{LeroyA_08a}
{Leroy}, A.K., {Walter}, F., {Brinks}, E., et al. 2008, \aj, 136, 2782 

\bibitem[Lilly et al.(2013)]{LillyS_13a}
{Lilly}, S.J., {Carollo}, C.M., {Pipino}, A., {Renzini}, A., \& {Peng}, Y. 2013, \apj, 772, 119 

%\bibitem[Lockman(2017)]{LockmanJ_Springer}
%{Lockman}, J.: in {\it Gas Accretion onto Galaxies}, Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion onto nearby galaxies, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Lopez et al.(2002)]{LopezS_02a}
{Lopez}, S., {Reimers}, D., {D'Odorico}, S., \& {Prochaska}, J.X. 2002, \aap, 385, 778

\bibitem[Lynden-Bell(1975)]{Lynden-BellD_75a}
{Lynden-Bell}, D. 1975, {\it Vistas in Astronomy}, 19, 299 

\bibitem[McBride et al.(2009)]{McBrideM_09a}
{McBride}, J., {Fakhouri}, O., \& {Ma}, C. 2009, \mnras, 398, 1858 

\bibitem[Mo et al.(1998)]{MoH_98a}
{Mo}, H.J., {Mao}, S., \& {White}, S.D.M. 1998, \mnras, 295, 319 

\bibitem[Noeske et al.(2007)]{NoeskeK_07a}
{Noeske}, K.G., {Faber}, S.M., {Weiner}, B.J., et al. 2007, \apjl, 660, L47 

\bibitem[Noterdaeme et al.(2012)]{NoterdaemeP_12b}
{Noterdaeme}, P., {Petitjean}, P., {Carithers}, W.C., 2012, \aap, 547, L1 

\bibitem[Pagel \& Patchett(1975)]{PagelB_75a}
{Pagel}, B.E.J., \& {Patchett}, B.E. 1975, \mnras, 172, 13 

\bibitem[Peng et al.(2010)]{PengY_10a}
Peng, Y.j., Lilly, S.J., Kova{\v{c}}, K., 2010, \apj, 721, 193

\bibitem[Peng \& Maiolino(2014)]{PengY_14b}
{Peng}, Y.J., \& {Maiolino}, R. 2014, \mnras, 443, 3643 

\bibitem[P{\'e}roux et al.(2003)]{PerouxC_03a}
{P{\' e}roux}, C., {McMahon}, R.G., {Storrie-Lombardi}, L.J., \& {Irwin}, M.J. 2003, 
\mnras, 346, 1103

\bibitem[P{\'e}roux et al.(2013)]{PerouxC_13a}
{P{\'e}roux}, C., {Bouch{\'e}}, N., {Kulkarni}, V.P., \& {York}, D.G. 2013,
\mnras, 436, 2650 

\bibitem[P{\'e}roux et al.(2011)]{PerouxC_11a}
{P{\'e}roux}, C., {Bouch{\'e}}, N., {Kulkarni}, V.P., {York}, D.G., \& {Vladilo},
  G. 2011, \mnras, 410, 2237 

\bibitem[P{\'e}roux et al.(2012)]{PerouxC_12a}
{P{\'e}roux}, C., {Bouch{\'e}}, N., {Kulkarni}, V.P., {York}, D.G., \& {Vladilo},
  G. 2012, \mnras, 419, 3060

\bibitem[P{\'e}roux et al.(2014)]{PerouxC_14a}
{P{\'e}roux}, C., {Kulkarni}, V.P., \& {York}, D.G. 2014, \mnras, 437, 3144

\bibitem[P{\'e}roux et al.(2016)]{PerouxC_16a}
{P{\'e}roux}, C., {Quiret}, S., {Rahmani}, H., et al. 2016, \mnras, 457, 903

\bibitem[P{\'e}roux et al.(2017)]{PerouxC_17a}
Peroux, C., Rahmani, H., Quiret, S., et al. 2017, \mnras, xx, yy

\bibitem[Pichon et al.(2011)]{PichonC_11a}
{Pichon}, C., {Pogosyan}, D., {Kimm}, T., et al. 2011, \mnras, 418, 2493

\bibitem[Putman et al.(2009)]{PutmanM_09a}
{Putman}, M.E., {Peek}, J.E.G., {Muratov}, A., 2009, \apj, 703, 1486 

%\bibitem[Richter(2017)]{RichterP_Springer}
%{Richter}, P., in {\it Gas Accretion onto Galaxies}, 
%Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion onto the Milky Way, p.~xx.
%Springer International Publishing Switzerland (2017)

%\bibitem[Rubin(2017)]{RubinK_Springer}
%{Rubin}, K.: in {\it Gas Accretion onto Galaxies}, 
%Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion seen down-the-barrel, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Saintonge et al.(2016)]{SaintongeA_16a}
{Saintonge}, A., {Catinella}, B., {Cortese}, L., et al. 2016, \mnras, 462, 1749

\bibitem[Saintonge et al.(2013)]{SaintongeA_13a}
{Saintonge}, A., {Lutz}, D., {Genzel}, R., et al. 2013, \apj, 778, 2 

\bibitem[Schmidt(1963)]{SchmidtM_63a}
{Schmidt}, M. 1963, \apj, 137, 758 

\bibitem[Schroetter et al.(2015)]{SchroetterI_15a}
{Schroetter}, I., {Bouch{\'e}}, N., {P{\'e}roux}, C., et al. 2015,
\apj, 804, 83 

\bibitem[Schroetter et al.(2016)]{SchroetterI_16a}
{Schroetter}, I., {Bouch{\'e}}, N., {Wendt}, M. 2016, \apj, in press (arXiv:1605.03412)

\bibitem[Shen et al.(2013)]{ShenS_13a}
{Shen}, S., {Madau}, P., {Guedes}, J., et al. 2013, \apj, 765, 89 

\bibitem[Steidel(1995)]{SteidelC_95b}
{Steidel}, C.C., 
%{The Nature and Evolution of Absorption-Selected Galaxies}.
%\newblock In: G.~{Meylan} (ed.) 
in {\it QSO Absorption Lines}, ESO Astrophysics Symposia, p. 139. 
Springer-Verlag, Berlin, Germany (1995)

%\bibitem[Stewart(2017)]{StewartK_Springer}
%{Stewart}, K.: in {\it Gas Accretion onto Galaxies}, 
%Astrophysics and Space Science Library, vol.~vv, p.~xx,
%chap. Gas accretion and angu}lar momentum, p.~xx.
%Springer International Publishing Switzerland (2017)

\bibitem[Stewart et al.(2016)]{StewartK_16a}
{Stewart}, K., {Maller}, A., {O{\~n}orbe}, J., et al. 2016, ApJ, submitted, arXiv:1606.08524 

\bibitem[Stewart et al.(2013)]{StewartK_13a}
{Stewart}, K.R., {Brooks}, A.M., {Bullock}, J.S., et al. 2013, \apj, 769, 74 

\bibitem[Stewart et al.(2011a)]{StewartK_11a}
{Stewart}, K.R., {Kaufmann}, T., {Bullock}, J.S., et al. 2011a, \apjl, 735, L1 

\bibitem[Stewart et al.(2011b)]{StewartK_11b}
{Stewart}, K.R., {Kaufmann}, T., {Bullock}, J.S., et al. 2011b, \apj, 738, 39 

\bibitem[Tacconi et al.(2013)]{TacconiL_13a}
{Tacconi}, L.J., {Neri}, R., {Genzel}, R., et al. 2013, \apj, 768, 74 

\bibitem[Tomczak et al.(2016)]{Tomczak2016}
Tomczak, A.R., Quadri, R.F., Tran, K.V.H., et al. 2016, \apj, 817, 118 

\bibitem[van den Bergh(1962)]{vandenberghS_62a}
{van den Bergh}, S. 1962, \aj, 67, 486 

\bibitem[Whitaker et al.(2012)]{WhitakerK_12a}
Whitaker, K.E., van Dokkum, P.G., Brammer, G., Franx, M. 2012, \apjl, 754, L29

\bibitem[Whitaker et al.(2014)]{WhitakerK_14a}
Whitaker, K.E., Franx, M., Leja, J., et al. 2014, \apj, 795, 104

\bibitem[White \& Frenk(1991)]{WhiteS_91a}
{White}, S.D.M. \& {Frenk}, C.S. 1991, \apj, 379, 52 

\bibitem[Yun et al.(1994)]{YunM_94a}
{Yun}, M.S., {Ho}, P.T.P., \& {Lo}, K.Y. 1994, Nature, 372, 530

\bibitem[Zafar et al.(2013)]{ZafarT_13a}
{Zafar}, T., {P{\'e}roux}, C., {Popping}, A., et al. 2013, \aap, 556, A141 

\end{thebibliography}

